A Theory of Factors Affecting Continuous Experimentation (FACE)

Continuous experimentation (CE) is used by many companies with internet-facing products to improve their software based on user data. Some companies deliberately adopt an experiment-driven approach to software development while some companies use CE in a more ad-hoc fashion. The goal of the study is to identify factors that explain the variations in the utility and efficacy of CE between different companies. We conducted a multi-case study of 12 companies involved with CE and performed 27 interviewees with practitioners at these companies. Based on that empirical data, we then built a theory of factors at play in CE. We introduce a theory of Factors Affecting Continuous Experimentation (FACE). The theory includes three factors, namely 1) processes and infrastructure for CE, 2) the user problem complexity of the product offering, and 3) incentive structures for CE. It explains how these factors affect the effectiveness of CE and its ability to achieve problem-solution and product-market fit. Our theory can be used by practitioners to assess an organisation's potential for adopting CE, as well as, identifying factors which pose challenges in gaining value from CE practices. Our results also provide a starting point for further research on how contextual factors affect CE and how these may be mitigated.

==> x_guidelines.tex <==
\section{Guidelines to Practitioners for Conducting CE}
\label{sec_pp3:discussion_recommendations}
Based on FACE, we have derived guidelines for practitioners. The guidelines are given as a list of recommendations on state-of-the-art CE processes and infrastructure and on how to strive towards it. According to Stol and Fizgerald~\cite{stol2015theory}, theories are suited as a starting point to derive practitioner guidelines from. 

\subsection{State-of-the-art CE practice}

Industry leading companies have published information on their state-of-the-art CE processes or infrastructure, such as Microsoft~\cite{gupta2018anatomy}, Google~\cite{tang2010overlapping} and Facebook~\cite{feitelson2013development}. Compared to those, two of the cases in our study have achieved equally high levels of experimentation, \textit{cases D and G}. They conduct experiments frequently, on all parts of their software, on most software changes, and on business relevant metrics. CE is an important part of their software development process, they have shifted from a mindset of shipping features to an experiment-driven approach where only functionality that are proven to solve user and or business needs are delivered. They are able to affect both problem-solution fit and product-market fit with their experimentation.

The RIGHT process and infrastructure model by Fagerholm et al.~\cite{fagerholm2017right} serves as a recommended starting point for practitioners. RIGHT contain no conflicting information to the ones reported here but it does not reflect mature CE. We have observed the following additional aspects of mature \emph{processes and infrastructure}:
\begin{itemize}
    \item \emph{Prioritization} should be based on user data. Companies use scoring methods to quantitatively prioritize expected impact and difficulty of implementation. Both cases D and G use the Impact, Confidence, Ease (ICE) scoring model~\cite{ellis2017hacking} and use user data to base the numbers on; when possible.
    \item \emph{Feasibility analysis} of experiments should be done before experiments are conducted. Only companies with High experimentation expertise (cases A, D, I, and G) conduct this step. It could be as simple as checking how many users use a feature or it could be a power analysis to control false discovery rates~\cite{kohavi2009controlled}. There are similar methods for qualitative research as well~\cite{vasileiou2018characterising}.
    \item \emph{Rigorous analysis} should be conducted after quantitative experiments are completed. The cases with High expertise in CE  monitor statistical significance on multiple metrics of different types: sales metrics, user experience metrics, and computation performance metrics. The calculations are simple~\cite{kohavi2009controlled}, so there is no reason to ignore statistical significance (or effect sizes, or Bayesian alternatives). Proper qualitative analysis is performed at Case K only, with a transcription and coding process.
    \item \emph{Mixed-methods experiments} are in use at cases D and G, since quantitative and qualitative data complement each other well. Other companies use one or the other. Prototyping pre-deployment experiments can be evaluated qualitatively to pre-validate ideas and to find hypotheses on what to experiment on. Following up with post-deployment experiments give definitive proof. Though, it does require additional roles in the form of both user experience researchers and data scientists to conduct proper analysis of the results.
    \item \emph{Knowledge sharing} is encouraged at companies with Medium or High CE expertise and is especially important when the experimenters are in a stand-alone team. Knowledge can be shared, for example, in workshops, mails, or internal wiki. One of the strengths of an experiment-driven development method is the opportunity to create domain knowledge through rigorous research. That effort could go to waste if the knowledge obtained from experiments is not curated.
    \item \emph{Infrastructure} is extensively expanded at the cases with High CE expertise. The \emph{data infrastructure} should support telemetry on all parts of the software and on multiple types of user data and it should be stored in a way that it can be tracked to experiment groups. The \emph{experimentation platform} should support managing parallel experiments, making inquiries into results for different user segments or metrics, and segmentation of users in order to obtain high throughput of experiments. The \emph{competences} should cover the necessary roles of experimentation. In addition, all software engineers need to be trained in experimentation so that they can partake in CE.
\end{itemize}

\subsection{Reaching state-of-the-art CE}

The theory identified three factors at play in experimentation, data infrastructure, user problem complexity, and incentive structures. These factors represent hurdles that companies need to overcome to reach experiment-driven development. What follows is the strategies the companies in the study used to achieve efficient and effective CE, also in unfavorable company contexts.
%\rasmus{hur strukturera så det knyts an till faktorerna? }
\begin{itemize}
    \item \emph{Build processes and infrastructure gradually.} While some companies were able to get started and ramp up experimentation (cases A and to some degree B) due to prior investments in data infrastructure, we recommend starting with experimentation practice instead of infrastructure processes. Starting with experimentation is easy, but scaling to high frequency and extent of experimentation is very challenging. The knowledge obtained from continuous experimentation will be useful for continuously scaling up infrastructure too.
    \item \emph{Seize opportunities to pivot} to simplify what problem the software solves for users. Problem complexity severely limits the ability for experiment-driven development. Case D was able to pivot successfully and was able to change to an experiment-driven process. However, pivoting is likely a challenging endeavor. Failed examples of pivoting might go unnoticed because a likely outcome of a failed pivot is bankruptcy.
    \item \emph{Use qualitative methods} to experiment in contexts with high problem complexity. Qualitative experiments are much easier to implement since they do not require high numbers of users and hence no deployment and they do not require specifying a quantitative metric. Cases K and L are able to conduct CE by validating software changes using qualitative experiments.
    \item \emph{Find the right goal} to experiment on that is relevant for both business and users. Metrics are hard to specify since they should stand up to abuse from unintentional attempts to game it, i.e., an improvement in the metric should always result in positive business and user value. For example, clicks are easy to get more of by adding additional steps users must complete, but that results in a worse user experience. 
    Many case companies are only able to use user experience metrics (such as clicks) that can improve problem-solution fit. However, by targeting product-market fit both users' and business' value can be optimized for simultaneously. Companies should put effort into finding the right goal for them, for example by carefully using proxy metrics (see Section~\ref{sec_pp3:theory_definitions}), using qualitative methods, or by providing team goals.
   % \rasmus{connect with previous one}
    \item \emph{Provide incentives with team goal metrics} so that all software engineers are encouraged to start with experimentation and to allow them to take responsibility of the experimentation process. This is easy to implement when working with quantitative experiments since the developers are provided with the necessary tools for achieving  the goals. Cases A, D, I, and G all use team goals. For the companies that do not have the right incentive structures in place they can compromise with process oriented goals, such as goals with how many of new features they are able to evaluate with qualitative experiments, etc. 
    \item \emph{Be mindful of ethics} when providing strong incentives to individuals. Team goals should be set with collaboration between the teams and management to ensure it is good for business and users. For example, one of the experiments mentioned by E1 was to hide the pause subscription button in a menu which drastically improved the churn rate and revenue. This also highlights the need for knowledge sharing since other developers pointed out the questionable experiment.
\end{itemize}

